Measurements of gluon-gluon fusion and vector-boson fusion Higgs boson production cross-sections in the $H \to WW^{\ast} \to e\nu\mu\nu$ decay channel in $pp$ collisions at $\sqrt{s}=13$ TeV with the ATLAS detector

Higgs boson production cross-sections in proton-proton collisions are measured in the $H \to WW^{\ast} \to e\nu\mu\nu$ decay channel. The proton-proton collision data were produced at the Large Hadron Collider at a centre-of-mass energy of 13 TeV and recorded by the ATLAS detector in 2015 and 2016, corresponding to an integrated luminosity of 36.1 fb$^{-1}$. The product of the $H \to WW^{\ast}$ branching fraction times the gluon-gluon fusion and vector-boson fusion cross-sections are measured to be $11.4 ^{+1.2}_{-1.1} (\mathrm{stat.}) ^{+1.8}_{-1.7}(\mathrm{syst.})$ $\mathrm{pb}$ and $0.50 ^{+0.24}_{-0.22} (\mathrm{stat.}) \pm 0.17(\mathrm{syst.})$ $\mathrm{pb}$, respectively, in agreement with the Standard Model predictions.

==> Modification_HIGG-2016-07.tex <==
While we were performing few check on the future analysis, we found a small issue in the results with 36/fb. We noticed that the trigger scale factors were applied twice. 
This leads to an underestimation of the predicted yields and then an overestimation of the ggF signal strength. 
The ggF signal strength is affected by less than 1 sigma and a negligible impact is observed on the VBF signal strength. 
The current version contains the update of the tables, plots and results reflecting the fix on the trigger scale factor issue.
The changes implemented in the paper are the following:
--> Removed ``the'' in last sentence of abstract: ``in agreement with Standard Model predictions'';
--> line 6: hyphenate second-largest;
--> Replaced “q” and “q’ ” with “q_1,q_2,q_3 and q_4”;
--> Figure 1-6: updated to reflect the fix on the trigger scale factors;
--> Table 1: Remove MadGraph as alternative generator for VBF;
--> Added the HDecay version used, HDecay v6.50;
--> Page 3, second paragraph added an additional reference for the ggF MC sample;
--> Page 3, third paragraph added a second reference for HDecay;
--> Sec. 3, parag. 3, replaced ''SM'' with ''Standard Model (SM)'';
--> Sec. 3, parag. 5, line 4: and the Sherpa parton shower, hadronization, added “the”;
--> Sec. 3, parag. 5, added a sentence on the Higgs signal and the WW background;
--> p. 6, 11 lines from bottom: ``and the two leading leptons''; Added “the”;
--> 3 lines from bottom: ``event with VBF-like kinematics'';  Remove the “the”;
--> Captions to Figs 3, 4, 5, 6, 7, and 8: replaced ``predictions'' with ``modelled contributions'';
--> Fig. 5 removed the tick marks on the right-hand side of the plot;
--> Table 3: fix a typo in the Z/gamma* CR for Njets=1, ggF;  ;
--> Table 4-6: updated to reflect the fix on the trigger scale factors;
--> p. 10, paragraph 1;  We replaced the following sentence “The contribution of this background in the SRs and CRs is then obtained by scaling the number of events in the control samples by an extrapolation factor” with 
“ The contribution of this background in the SRs and CRs is then obtained by scaling the number of data events, after the subtraction of process with two prompt leptons,  in the control samples by an extrapolation factor”.
--> Sec 4, para 1: For muons, high efficiency. Replaced “For the muon” with “For muons”;
--> Sec 6: ``other sources of uncertainty ... criteria''; removed “criteria”;
--> Table 5 caption: ``yields in the ggF and VBF SRs.'', added the “the”;
--> Cross-sections and signal strengths updated to reflect the fix on the trigger scale factors;
--> Description of Table 6 in section 7 has been update to reflect the above changes;
--> Figure 9: Fixed labels in the legend;  
--> Last sentence of conclusion: ``... in agreement with SM predictions.''; removed “the”, and replacec ''Standard Model'' with SM.



